Alternative Speech: Complementary Method to Counter-Narrative for Better Discourse

We introduce the concept of "Alternative Speech" as a new way to directly combat hate speech and complement the limitations of counter-narrative. An alternative speech provides practical alternatives to hate speech in real-world scenarios by offering speech-level corrections to speakers while considering the surrounding context and promoting speakers to reform. Further, an alternative speech can combat hate speech alongside counter-narratives, offering a useful tool to address social issues such as racial discrimination and gender inequality. We propose the new concept and provide detailed guidelines for constructing the necessary dataset. Through discussion, we demonstrate that combining alternative speech and counter-narrative can be a more effective strategy for combating hate speech by complementing specificity and guiding capacity of counter-narrative. This paper presents another perspective for dealing with hate speech, offering viable remedies to complement the constraints of current approaches to mitigating harmful bias.

==> tables/1.exam_as.tex <==
\begin{table*}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\scalebox{0.78}{
\begin{tabular}{p{1.2cm}p{7.7cm}}
\toprule
  Hate-speech &
  \begin{tabular}[c]{p{7.6cm}}
  (a) Islamic are criminals: they rape, enslave and murder people. Islam is more a worship than a religion and we do not have anything to share with them. \\ \\ 
  (b) Muslims should not exist in our modern world, because all that they do is violence.\\ \\ (c) Islam is not a religion, its just an excuse for retarded sexual psychopaths, bastards who pollute the world.
  \end{tabular} & 
\midrule
  Counter-narrative &
  \begin{tabular}[c]{p{7.6cm}}
  People have the right to belong to any religion they want. If you do not like their religion, it does not mean that they are bad!
  \end{tabular} &
\midrule
  Alternative speech &
  \begin{tabular}[c]{p{7.6cm}}
  (a) Islamic are ordinary people: they embrace and get along with people. Islam is more of a general religion, not worship, and we have a lot to share with them.\\ \\ 
  (b) Muslims are necessary in our modern world, because they play an important role in various places.\\ \\ 
  (c) Islam is a religion and does not pollute the world.
  \end{tabular} &
\bottomrule
\end{tabular}
}
\caption{Examples of counter-narrative and alternative speech for hate speech. Given hate speech and counter-narrative are extracted from the CONAN dataset~\cite{chung2019conan}.}
\label{tab:exam_as}
\end{table*}

==> tables/2.more_ex.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[ht]
\centering
\renewcommand{\arraystretch}{1.2}
\scalebox{0.78}{
\begin{tabular}{p{3cm}|p{5cm}|p{5cm}|p{6cm}}
\toprule
  Dataset &
  HS &
  AS &
  CN &
\toprule
   &
  (a) Islam looks like a cult more than like a religion. It is beliefs make people rape children and commit violence. It should not be accepted in our country. &
  (a) Islam is a religion more than a cult. It is beliefs make people respect children and follow the rules. It should be embraced in our country. &
   & \cline{2-3}
  \multirow{3}{*}{\citet{chung2019conan}} &
  (b) I am done with Islam and isis. All Muslims should be sent to their homeland. Britain will be better without their violence and ideology &
  (b) I acknowledge Islam. All Muslims possess the right to reside in the place of their choice. Britain will be better with their peace and ideology. &
  The world would actually be a very dark place without Muslims who contribute a lot to our society. What about our Muslim, doctors, scientists, philanthropists, actors, job-creators. &
\cline{2-3}
   &
  (c) Everything will be better if Muslims did not exist. Their only contribute to our society is violence. &
  (c) Nothing will be change if Muslims exist. Their contribute to our society is found in various aspects. &
   \\
\midrule
  &
  (a) Downies are just sick people that can't integrate into society because of their disease. &
  (a) Downies are just sick people that should not be excluded from society just because of their disease. &
  & \cline{2-3}
  \multirow{3}{*}{\citet{fanton2021human}} &
  (b) Children with Down Syndrome may hinder the development process of other children. They should be isolated. &
  (b) Children with Down Syndrome may help the development process of other children. They should be grown together. &
  Coexisting and studying with handicapped children helps develop sensitivity, insight and understanding &
\cline{2-3}
 &
  (c) Downy children should be isolated in special schools for their own interest. &
  (c) Downy children should have an opportunity to choose schools for their own interest. &
   &
\midrule
  &
  (a) Children should learn about gender identity and sexual orientation from their families rather than in class from LGBT fundamentalist. &
  (a) Children should learn about gender identity and sexual orientation from their families and classes. &
  & \cline{2-3}
  \multirow{3}{*}{\citet{chung-etal-2021-towards}} &
  (b) We should restrain from imposing gender ideology on children. &
  (b) We should be careful with imposing gender ideology on children. &
  If gender identity is taught to foster nondiscrimination policy and parents are indeed able to opt out of those classes, what is the problem? &
  \cline{2-3}
  & 
  (c) LGBTs just want to brainwash our children. They should not be taught about gender identity and sexual orientation in school. &
  (c) LGBTs just want to be understood by our children. They should be taught about gender identity and sexual orientation in school. &
   &
\bottomrule
\end{tabular}
}
\caption{}
\label{tab:more_ex}
\end{table*}
